$\tau$-tilting theory: a self-contained introduction

A self-contained introduction to the basics of Tau-tilting theory. We assume that the reader is familiar with Auslander-Reiten theory, but circumvent the need for the Brenner-Butler tilting theorem completely.

==> preamble.tex <==
\usepackage[left=1in, right=1in, top=1in, bottom=1in, includefoot, headheight=14.5pt]{geometry}

\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhead[L,C]{}
\fancyhead[L]{\nouppercase{\leftmark}}
\fancyhead[R]{\rightmark}
\fancyfoot[C]{\thepage}

%packages
\usepackage{amsmath} % Standard math package by the American Mathematical Society
\usepackage{amsthm} % Necessary so that \newtheorem* works. To make package cleveref work
\usepackage{amssymb, mathtools} % Not sure why these are useful yet. amssymb adds commonly used math symbols

\usepackage{enumitem} % Better than enumerate
\setlist[enumerate, 1]{label=\arabic*)}

\usepackage{tikz-cd} % Tools for drawing communitative diagrams

\RequirePackage{mathpazo} % (they're just palatino fonts but open-source and in the case of mathpazo, mathified)
\usepackage{charter} % Charter for text. The math symbols from mathpazo are still there.

\usepackage{parskip} % No indents for paragraphs, instead slightly more vertical spacing 

\usepackage{booktabs} % Required to use pandas.DataFrame.to_latex.

\usepackage{tcolorbox} % provides colored boxes for framed math environments

\usepackage{diagbox} % diagonal slash in corner of table
\usepackage{adjustbox} % adjust size of table which is too wide, and centering it properly


\usepackage{array} % Create arrays
\usepackage[marginpar]{todo}

\usepackage[bookmarksopen=true,bookmarks=true]{hyperref} %Make sure it comes last of your loaded packages, to give it a fighting chance of not being over-written, since its job is to redefine many Latex commands
\usepackage{bookmark}
\usepackage{aliascnt} % see \sharedtheorem below

\usepackage{cleveref}

% PREAMBLE: GENERAL MATHEMATICS
\newtheoremstyle{definition}% 〈name〉
{}% 〈Space above〉1
{}% 〈Space below 〉1
{}% 〈Body font〉
{}% 〈Indent amount〉2
{\bfseries}% 〈Theorem head font〉
{:}% 〈Punctuation after theorem head 〉
{\newline}% 〈Space after theorem head 〉3
{}% 〈Theorem head spec (can be left empty, meaning ‘normal’ )

\newtheoremstyle{plain}% 〈name〉
{}% 〈Space above〉1
{}% 〈Space below 〉1
{\itshape}% 〈Body font〉
{}% 〈Indent amount〉2
{\bfseries}% 〈Theorem head font〉
{:}% 〈Punctuation after theorem head 〉
{\newline}% 〈Space after theorem head 〉3
{}% 〈Theorem head spec (can be left empty, meaning ‘normal’ )

% All numbered environments share the definition counter. Each one gets its
% own alias of that counter, since otherwise cleveref (on TeX Live 2025 and
% later) names every reference after the shared counter, ie. "definition 1.3"
% for a proposition.
\newcommand{\sharedtheorem}[2]{%
    \newaliascnt{#1}{definition}%
    \newtheorem{#1}[#1]{#2}%
    \aliascntresetthe{#1}%
    \newtheorem*{#1*}{#2}%
}

\theoremstyle{definition} %definition
\newtheorem{definition}{Definition}[section]
\newtheorem*{definition*}{Definition}

\sharedtheorem{example}{Example}
\sharedtheorem{remark}{Remark}
\sharedtheorem{notation}{Notation}

\theoremstyle{plain}
\sharedtheorem{theorem}{Theorem}
\sharedtheorem{corollary}{Corollary}
\sharedtheorem{lemma}{Lemma}
\sharedtheorem{proposition}{Proposition}
\sharedtheorem{conjecture}{Conjecture}
\sharedtheorem{question}{Question}

%custom defined math operators
\DeclareMathOperator{\Mod}{\!-mod}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Ext}{Ext} 
\DeclareMathOperator{\Tor}{Tor} 
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\Fun}{Fun}

\DeclareMathOperator{\fac}{fac}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\gen}{gen}
\DeclareMathOperator{\cogen}{cogen}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\projdim}{proj.dim}
\DeclareMathOperator{\injdim}{inj.dim}
\DeclareMathOperator{\mh}{`\-}
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\trans}{Tr}
\DeclareMathOperator{\ann}{ann}
\DeclareMathOperator{\supportrank}{srank}
\DeclareMathOperator{\rank}{rk}
\DeclareMathOperator{\rad}{rad}


\newcommand{\ii}{\item}
\newcommand{\op}{^{\text{op}}}

%Script letters: mathcal > mathscr	 
\newcommand{\SA}{\mathcal A}
\newcommand{\SB}{\mathcal B}
\newcommand{\SC}{\mathcal C}
\newcommand{\SD}{\mathcal D}
\newcommand{\SE}{\mathcal E}
\newcommand{\SF}{\mathcal F}
\newcommand{\SG}{\mathcal G}
\newcommand{\SH}{\mathcal H}
\newcommand{\SI}{\mathcal I}
\newcommand{\SJ}{\mathcal J}
\newcommand{\OO}{\mathcal O}
\newcommand{\SP}{\mathcal P}
\newcommand{\SR}{\mathcal R}
\newcommand{\SSS}{\mathcal S}
\newcommand{\ST}{\mathcal T}
\newcommand{\SX}{\mathcal X}
\newcommand{\SY}{\mathcal Y}



%The following ones are custom ones taken from Evan Chen's Napkin. 
%Not all were taken, just some that seemed useful.
%https://github.com/vEnhance/napkin/blob/main/tex/macros.tex
\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}

%From H113 "Introduction to Abstract Algebra" at UC Berkeley
\newcommand{\BA}{\mathbb A}
\newcommand{\CC}{\mathbb C}
\newcommand{\FF}{\mathbb F}
\newcommand{\NN}{\mathbb N}
\newcommand{\QQ}{\mathbb Q}
\newcommand{\RR}{\mathbb R}
\newcommand{\ZZ}{\mathbb Z}


%From Kiran Kedlaya's "Geometry Unbound"
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}


\newcommand{\id}{\mathrm{id}}
\newcommand{\inv}{^{-1}}
%% End of Evan chen macros

%Function restriction: This is (obviously) from the Stackexchange post
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

% PREAMBLE: TAU-TILTING THEORY

\newcommand{\ta}{$\tau$}
%\newcommand{\stt}{s \tau - tilt (A)}
%\newcommand{\fft}{f \mh tors (A)}
\newcommand{\transpose}{\text{Tr }}
\newcommand{\dualpr}{_{\text{pr}}}
\newcommand{\dualnp}{_{\text{np}}}

% Adachi, Iyama, Reiten, \ta-tilting theory
\newcommand{\tors}{\mbox{\rm tors}\hspace{.01in}}
\newcommand{\ftors}{\mbox{\rm f-tors}\hspace{.01in}}
\newcommand{\sftors}{\mbox{\rm sf-tors}\hspace{.01in}}
\newcommand{\fftors}{\mbox{\rm ff-tors}\hspace{.01in}}

\newcommand{\sttilt}{\mbox{\rm s$\tau$-tilt}\hspace{.01in}}
\newcommand{\psttilt}{\mbox{\rm ps$\tau$-tilt}\hspace{.01in}}
\newcommand{\ttilt}{\mbox{\rm $\tau$-tilt}\hspace{.01in}}
\newcommand{\tilttilt}{\mbox{\rm tilt}\hspace{.01in}}

\newcommand{\trigid}{\mbox{\rm $\tau$-rigid}\hspace{.01in}}
\newcommand{\tminusrigid}{\mbox{\rm $\tau^-$-rigid}\hspace{.01in}}
\newcommand{\sminusttilt}{\mbox{\rm s$\tau^-$-tilt}\hspace{.01in}}
\newcommand{\bong}{{}^{\perp 0}}

\newcommand{\fbrick}{\mbox{\rm f-brick}\hspace{.01in}}

% General AR-theory stuff:
% Dimension vectors for AR-quivers. Just a small matrix with two, respectively three rows. 
\newcommand{\ind}[2]{%
	\begin{smallmatrix}#1\\#2\end{smallmatrix}%
}
\newcommand{\indd}[3]{%
	\begin{smallmatrix}#1\\#2\\#3\end{smallmatrix}%
}
% TIKZCD The (inverse) auslander reiten translate. This goes two steps two the right, which should work for most knitted quivers.
\newcommand{\art}{\ar[rr, dashed, "\tau^{-}" description]}

